Predicting User Experience on Laptops from Hardware Specifications

Estimating the overall user experience (UX) on a device is a common challenge faced by manufacturers. Today, device makers primarily rely on microbenchmark scores, such as Geekbench, that stress test specific hardware components, such as CPU or RAM, but do not satisfactorily capture consumer workloads. System designers often rely on domain-specific heuristics and extensive testing of prototypes to reach a desired UX goal, and yet there is often a mismatch between the manufacturers' performance claims and the consumers' experience. We present our initial results on predicting real-life experience on laptops from their hardware specifications. We target web applications that run on Chromebooks (ChromeOS laptops) for a simple and fair aggregation of experience across applications and workloads. On 54 laptops, we track 9 UX metrics on common end-user workloads: web browsing, video playback and audio/video calls. We focus on a subset of high-level metrics exposed by the Chrome browser, that are part of the Web Vitals initiative for judging the UX on web applications. With a dataset of 100K UX data points, we train gradient boosted regression trees that predict the metric values from device specifications. Across our 9 metrics, we note a mean $R^2$ score (goodness-of-fit on our dataset) of 97.8% and a mean MAAPE (percentage error in prediction on unseen data) of 10.1%.

==> sections/conclusion.tex <==
\section{Conclusion \& Future Work}%
\label{sec:conclusion}

In conclusion, we present an ML approach for predicting
the user experience (UX) on Chromebook laptops across real-life workloads.
Prior work focuses on predicting microbenchmark scores,
which do not satisfactorily model the overall UX on real-life consumer workloads.
We identify a set of key UX metrics within the Chrome browser,
and define test workloads over common end-user use cases seen in telemetry data.
On this dataset, we train gradient boosted regression trees,
that accurately predict the UX metric values
given the hardware specifications for a Chromebook.

Our promising initial results open the door for several interesting future work.
The first step is to expand our workloads
to also include non-native (Linux and Android) applications.
These applications within virtual machines (VMs) or containers in ChromeOS,
and would thus require significant changes
to our test automation and metric collection stack.
Another direction is to compare UX when the devices are running on battery,
when their performance is usually throttled to conserve power.
One approach would be to introduce a new input to our current models,
for battery status -- charging or discharging.
Finally, we believe this methodology can be extended to devices beyond Chromebooks.
With sufficient data about end-user workloads on Windows, Mac, and Linux devices,
we should be able to train similar models to predict user experiences on these devices as well.

